Dumbo-NG: Fast Asynchronous BFT Consensus with Throughput-Oblivious Latency

Despite recent progresses of practical asynchronous Byzantine fault tolerant (BFT) consensus, the state-of-the-art designs still suffer from suboptimal performance. Particularly, to obtain maximum throughput, most existing protocols with guaranteed linear amortized communication complexity require each participating node to broadcast a huge batch of transactions, which dramatically sacrifices latency. Worse still, the f slowest nodes' broadcasts might never be agreed to output and thus can be censored (where f is the number of faults). Implementable mitigation to the threat either uses computationally costly threshold encryption or incurs communication blow-up, thus causing further efficiency issues. We present Dumbo-NG, a novel asynchronous BFT consensus (atomic broadcast) to solve the remaining practical issues. Its technical core is a non-trivial direct reduction from asynchronous atomic broadcast to multi-valued validated Byzantine agreement (MVBA) with quality property. Most interestingly, the new protocol structure empowers completely concurrent execution of transaction dissemination and asynchronous agreement. This brings about two benefits: (i) the throughput-latency tension is resolved to approach peak throughput with minimal increase in latency; (ii) the transactions broadcasted by any honest node can be agreed to output, thus conquering the censorship threat with no extra cost. We implement Dumbo-NG and compare it to the state-of-the-art asynchronous BFT with guaranteed censorship resilience including Dumbo (CCS'20) and Speeding-Dumbo (NDSS'22). We also apply the techniques from Speeding-Dumbo to DispersedLedger (NSDI'22) and obtain an improved variant of DispersedLedger called sDumbo-DL for comprehensive comparison. Extensive experiments reveal: Dumbo-NG realizes better peak throughput performance and its latency can almost remain stable when throughput grows.

==> Preliminaries.tex <==
%!TEX root = main.tex
\section{Notations and Preliminaries}

%We introduce definitions for some underlying building blocks.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\smallskip\noindent{\bf Reliable broadcast ($\mathsf{RBC}$)} is a protocol running among a set of $n$ nodes \cite{bracha1987asynchronous} in which there is a node called sender whose aim is to broadcast a value to all the other nodes. More formally, an $\mathsf{RBC}$ protocol satisfies the following properties:

\begin{itemize}
	\item {\em Agreement}. If two honest nodes delivers $ v $ and $v'$ respectively, then $ v = v'$;
	
	\item {\em Totality}. If an honest node delivers $ v $, then all honest nodes deliver $ v $;
	
	\item {\em Validity}. If the sender is honest and inputs $ v $, then all honest nodes deliver $ v $.
\end{itemize}

% In an $\mathsf{RBC}$ protocol, erasure code as well as merkle-tree are adopted to reduce the communication cost of input requirement.  Besides, 
 
Remark: throughout the paper, we adopt a $(\left \lceil \frac{n+1}{3} \right \rceil,n)$-erasure code scheme in $\mathsf{RBC}$. {\bf Consistent broadcast} ($\mathsf{CBC}$) is similar to RBC, but it does not provides {\em Totality}. Please see Appendix  for details of some concrete constructions of $\mathsf{RBC}$ and $\mathsf{CBC}$ protocols. %\qiang{unclear}



\noindent{\bf Asynchronous binary agreement ($\mathsf{ABA}$)} is a special asynchronous Byzantine agreement protocol among $n$ nodes \cite{mostefaoui2014signature}. In an $\mathsf{ABA}$ protocol, each node has a single-bit (0/1) input, and their goal is to reach an agreement on the output bit. More formally, an $\mathsf{ABA}$ protocol has the following guarantees:

\begin{itemize}
	\item {\em Agreement}. If any honest node outputs the bit $ b $, then every honest node outputs $ b $;
	
	\item {\em Termination}. If all honest nodes receive input, then every honest node outputs a bit;
	
	\item {\em Validity}. If any honest node outputs $ b $, then at least one honest node received $ b $ as input.
\end{itemize}

}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent \textbf{Notations}. 
Through the paper, we let $|m|$ be the bit-length of protocols' input,
$\lambda$ be the cryptographic security parameter that captures the size of (threshold) signature and the length of hash value. 
$\hash$ denotes a collision-resistant hash function. %$\{0,1\} ^ {*} \rightarrow \{0,1\} ^ \lambda$.
%$\TSIG$ denote threshold signature  and  threshold encryption, respectively. 
We also consider established threshold signature consisting of a tuple  of algorithms $(\SignShare_t, \VerifyShare_t,\Combine_t, \Verify_t)$, where the subscript $t$ in notations represents threshold, cf. Appendix \ref{app:tsig} for the syntax and securities of the primitive.
%, cf. for their syntax and security definitions in Appendix \yuan{??? The for formal definitions and implementation details can be found in the full paper \cite{??}.}.
%
%
%
%
A protocol message has a syntax of $(\mathsf{MsgType}, \DID, \cdots)$, where $\mathsf{MsgType}$ defines the message type and  $\DID$  is the session identifier representing a specific protocol instance.   
%
%The pseudocode of our protocol   follows the conventional way to describe asynchronous protocols \cite{cachin01,ittai19,lu2020dumbo}: we let ``{\em wait for}'' to represent that the protocol is blocking until a certain event; sometimes, we omit an implicit ``{\em wait for}'' handler for   the incoming messages and use ``{\em upon receiving}'' to describe how to process  an applicable message; ``{\em multicast}'' means to send a message to all nodes; ``{\em output}'' means to return some value without halt; %``{\em return W}'' means to output {\em W} and then halt;
Moreover, $\Pi[\DID]$ represents an instance of some protocol $\Pi$ with a session identifier $\DID$, and $y\leftarrow\Pi[\DID](x)$ means to invoke $\Pi[\DID]$ on input $x$ and wait for its  output $y$.
Sometimes, $\Pi[\DID](x)$ itself also denotes the protocol output  for brevity.
%
Also, $\langle x, y \rangle$   denotes a string concatenating  two strings $x$ and $y$.



\noindent \textbf{Multi-valued validated Byzantine agreement ($\mathsf{MVBA}$)} \cite{abraham2018validated,cachin2001secure} 
is a variant of Byzantine agreement with external validity, such that the participating nodes can agree on a value satisfying  a global and polynomial-time computable predicate $Q$ known by all of them (which can be concretely specified due to the application scenarios). 
Syntax-wise, each node in the protocol would take a (probably different) value validated by the predicate $Q$  as input and can decide  a common value satisfying $Q$ as the output. 
%The protocol ensures that the decision value was proposed by at least one node. All honest node only input a value to $\mathsf{MVBA}$ that satisfy $Q$. 
%In this paper, we consider $W=\{ (s_1,\sigma_1),  (s_2,\sigma_2),\cdots, (s_n,\sigma_n)\}$ as the input of $\mathsf{MVBA}$. The predicate $Q$ require at least $n-f$ distinct $i$ satisfy $s_i\neq \perp $ in $W$, and for each value $(s_i,\sigma_i)$ of $W$, $\sigma_i$ satisfy the signature verification algorithm $\mathsf{Verify}_{f+1}$ if $s_i\neq \perp $.

The protocol (with an explicit predicate $Q$) shall satisfy the following properties except with negligible probability:
	\begin{itemize}
		\item {\em Termination.} If all honest nodes are activated on an identifier $\DID$ with taking as input some values satisfying $Q$, then each honest node would output a value for $\DID$;
		
		\item {\em External-Validity.} If an honest node outputs a value $v$ for some $\DID$, then $v$ is valid for $Q$, i.e., $Q(v) = 1$;
		
		\item {\em Agreement.} All honest nodes would decide the same value as output for the same $\DID$.
		
		
	\end{itemize}



\noindent \textbf{Leader election} % from the $(n,t)$ threshold signature} 
($\IDE$) is a protocol   among $n$ nodes that can output an unpredictable index representing a node in the system. 
It satisfies the following properties with an overwhelming probability:

\begin{itemize}
    \item {\em Termination:} If all honest nodes activate the protocol on an identifier $\DID$, each honest node would output some index $\ell \in [n]$ for $\DID$;
    \item {\em Agreement:} All honest nodes would output the same index $\ell$ for the same $\DID$; 
    \item {\em Unpredictability:} Before $t-f$ nodes invoke the protocol on an identifier $\DID$ (where $f$ represents the number of corrupted nodes), 
    no node can successfully predicate the output for $\DID$ except with $1/n$ probability (i.e., no better than guessing from $[n]$).
\end{itemize}

The $(n,t)$ $\IDE$ protocol can be instantiated by $(n,t)$ non-interactive threshold (unique) signature under setup assumptions in the random oracle model \cite{cachin2000random}. 
The details of the classic construction is illustrated in Alg. \ref{ce} in Appendix \ref{app:elect}.

\noindent{\bf Provable broadcast} ($\pcbc$, adapted from \cite{abraham2018validated})
is a broadcast protocol among $n$ nodes with a designated node called sender and a global predicate function $\ValidateVal$ for validating the sender's input.
The sender takes a tuple $m:=(v,\pi)$ as input, where $v$ is a value and $\pi$ is a string to validate $v$ according to $\ValidateVal$.
Then, each node would output a tuple $value:=(v, \pi)$. The sender additionally outputs a tuple $lock:=(h, \sigma)$, where $h$ is the hash of some value $v$ and $\sigma$ is a threshold signature that aggregates $2f+1$ signature shares for $h$. In addition, each node can invoke an $abandon$ interface during the execution to quit from the protocol.
%
%Specifically,  the sender returns an additional proof $\sigma $ by a $\mathsf{Proof}$ message. Informally, $\sigma$ proves, via the threshold signature abstraction, that at least $f+1$ honest nodes delivered same value from the sender by a $\mathsf{Value}$ message. Besides, if the sender produce two valid proofs $\sigma $ and proof $\sigma'$, then $\sigma=\sigma'$ %We do some light revise which is due to the API of our $\pcbc$ broadcasts somewhat differs from Abraham et al. \cite{abraham2018validated} 
\footnote{Different from \cite{abraham2018validated}, here we consider the threshold signature for the hash value of the message instead of for the message itself, which is a natural extension in the presence of collision-resistance hash function and later might save communications when we leverage the provability to construct more efficient MVBA.
%, the input of MVBA is some small size values, and also can verify its validation at the same time, e.g.  message' indexes, hash value and some proofs, where the proof corresponds to the indexes and hash value
} 

Besides the above syntax, a $\pcbc$ protocol with a session identifier $\DID$ satisfies the next properties with all but negligible probability:

\begin{itemize}
    \item {\em Validity}. If any honest $\node_i$ outputs  a tuple ${value}:=(v,\pi)$, then $\ValidateVal(\DID,(v,\pi)) = 1$.
    %the input will be reject unless $\ValidateVal(\DID,m) = true$.
 
	\item {\em Termination}. %If the sender is honest and inputs $v$, then all honest nodes deliver $v$; additionally, the sender outputs a proof $\sigma$ which satisfies $\Verify_{(2f+1)}(\ID, h(v),\sigma)=1$. 
	If the sender $\node_s$ is honest and inputs $m:=(v,\pi)$ satisfying $\ValidateVal(\DID,m) = 1$ and all honest nodes activate $\pcbc[\DID]$ without invoking $abandon(\DID)$,  %and the message $m:=(v,\prf)$ that is being broadcast is externally valid, i.e. $\ValidateValue(\ID,m) = 1$,
	then all honest nodes would output ${value}:=m$; additionally, the sender outputs a 
	tuple $lock:=(h, \sigma)$, where $h=\hash(v)$ and $\Verify_{(2f+1)}(\DID, h,\sigma)=1$. 

	\item {\em Provability}. % For any two valid $m=(v,\pi)$ and $m'=(v',\pi')$, i.e., $\ValidateVal(\DID,m) = 1$ and $\ValidateVal(\DID,$ $m')$ $ = 1$
	If the sender can produce $lock:=(h, $ $ \sigma)$ and $lock':=(h', \sigma')$ s.t. $\Verify_{(2f+1)}(\DID, h, \sigma)=1$ and $\Verify_{(2f+1)}$ $(\DID,h',\sigma')=1$, then (1) $h=h'$ and (2) at least $f+1$ honest nodes output ${value}:=(v, \pi)$ satisfying that $\hash(v)=h$ and  $\ValidateVal(\DID, value) = 1$.
	
%	\item {\em Integrity}. An honest node delivers a message at most once.
    
    \item {\em Abandon-ability}. An honest node does not deliver any message associated to $\DID$ after it invokes $abandon(\DID)$.
   
\end{itemize}

A  construction of $\pcbc$ is deferred to Alg. \ref{algPB} in Appendix \ref{app:pb}, which costs only $\bigO(1)$ time, $\bigO(n)$ messages, and $\bigO(|m| n+\lambda n)$ bits.







==> algorithm.tex <==
%!TEX root = main.tex

%\section{A Broadcast-with-consensus Protocol}












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\begin{figure*}[htbp]
\begin{small}
	\begin{tcolorbox}[
			colframe=gray!15,
			colback=gray!5,
			coltitle=gray!25!black,  
			fonttitle=\bfseries,
			adjusted title=The {\em $\xdumbo$} protocol (for each party $\node_i$)]

\textbf{let} $\buf$ to be a FIFO queue of input transactions, $B$ to be the batch size parameter %,  $\sigma_{i,0}=\bot$ for all $1\leq i\leq n$

\textbf{initial} $\heights := [({\height}_1,\digest_1,\Sigma_{1}), \dots, ({\height}_n,\digest_n,\Sigma_{n})]$ 
as $[(0 , \bot, \bot), \dots, (0 , \bot, \bot)]$  

for every $j\in[n]$, \textbf{initial} $\blocks[j]$ as an empty list

\vspace{2mm}
Each node $\node_i$ runs the protocol %in consecutive slot numbered $s$ (initialized as 1) 
consisting of next processes:



 	\vspace{2mm}
	\textbf{Payload Proposal} (a process). %for each $\node_i$:
	\begin{itemize}
		\item \textbf{initial} $\Sigma \leftarrow \bot$								
		\item		\textbf{for} each slot $s\in\{1,2,3,\dots\}$: %for $s=1,2,3,\cdots$ %if $s > 1$ then: 
		\begin{itemize}
		\item $\payload \leftarrow \buf[:B]$,
		$\digest \leftarrow \hash(\payload)$,
		\textbf{multicast} $\proposal(s, \payload,\Sigma)$ 						
		%\Comment{ $\payload_{i,s}$ is $\node_i$ sent in slot $s$ }					
			%\item wait for $2f+1$ $\vote(i, s-1,\rho_{s-1,j})$ from distinct parties $\node_j$, where $\VrfyShare_{2f+1}(\langle i, s-1, \hash(\payload_{i,s-1}) \rangle,$ $(j,\rho_{s-1,j})) =1$, then compute $\sigma_{i,s-1} \leftarrow\Combine_{2f+1}( \langle i, s-1, \hash(\payload_{i,s-1}) \rangle,\{(j, \rho_{s-1,j})\}_{2f+1} )$, 	$s\leftarrow s+1$	
		\item \textbf{wait for} $2f+1$ $\vote(s,\sigma_{j,s})$ from distinct nodes $\{\node_j\}$ s.t. $\VrfyShare_j( i||s||\digest,\sigma_{j,s}) = \true$:
		\begin{itemize}
			\item $\Sigma \leftarrow\Combine(  i||s||\digest,\{(j, \sigma_{j,s})\}_{j\in\{\node_j\}} )$
		\end{itemize}
		%where $\VrfyShare_j( i||s||\hash(\payload_{i,s}) ,\rho_{s,j}) =1$, then compute $\sigma_{i,s} \leftarrow\Combine_{2f+1}( \langle i, s, \hash(\payload_{i,s}) \rangle,\{(j, \rho_{s,j})\}_{2f+1} )$, $s\leftarrow s+1$							
		\end{itemize}					
 	\end{itemize}					
	
 	\vspace{2mm}
	\textbf{Payload Vote and Deliver} ($n$ processes). 
	\begin{itemize}
		\item \textbf{for} each  $j\in[n]$, {start a process as follows}:
		\begin{itemize}
			%\item let $\sigma^j_{0} \leftarrow \bot$
			%\item start a process (to handle $\node_j$'s proposals) as follows
			\item \textbf{for} each slot $s\in\{1,2,3,\dots\}$: %for $s=1,2,3,\cdots$ %if $s > 1$ then:
			\begin{itemize}
				\item upon receiving    $\proposal(s, \payload_{j},\Sigma_{j,s-1})$ from $\node_j$ for the first time:
				\begin{itemize}
					\item record $\blocks[j][s]\leftarrow \payload_{j}$,
					record $\digest_{j,s} \leftarrow \hash(\payload_{j,s})$
					\item if $s>1$ and $\Vrfy( j||s-1||\digest_{j,s-1}, \Sigma_{j,s-1})$:
					\begin{itemize}
						%\item deliver $\blocks[j][s]:=(\payload^j_{s-1}, \prf^{j}_{s-1})$, where $\prf^{j}_{s-1}:=(\digest^j_{s-1}, \sigma^j_{s-1})$
						%\item deliver $\blocks[j][s]:= \payload^j_{s-1}$															
						\item  $(\height_j, \digest_j, \Sigma_j) \leftarrow (s-1 , \digest_{j,s-1}, \Sigma_{j,s-1})$ %, where $(\height_j,\Sigma_j)$ is the $j$-th element in  $\heights$
					\end{itemize}									
					\item  compute $\sigma_{s} \leftarrow \SignShare_i(j||s||\digest_{j,s})$, send $\vote(s, \sigma_{s})$ to $\node_j$
				\end{itemize}
			\end{itemize}
		\end{itemize}

	\end{itemize}

	 	\vspace{2mm}
	\textbf{Consensus for Ordering Payloads}  (a process). 


%\vspace{-0.2cm}				
%\hrulefill
		 


	\begin{itemize}
	\item \noindent \textbf{initial} $\agreeds:=[\agreed_1,\dots,\agreed_n]$ as $[0,\dots,0]$ %where $\agreed_j \leftarrow 0$ for each $j\in[n]$; %$M_i=\{ (H^1,b_i^1,m_i^1),\cdots, (H^n,b_i^n,m_i^n)\}$, where $(H^j,b_i^j,m_i^j) \leftarrow (\perp, \perp, \perp)$ for all $1\leq j\leq n$; ${HS} \leftarrow \emptyset$; $FS = 0$; $Ready = false$.
	\item \textbf{for} each slot $s\in\{1,2,3,\dots\}$:
	\begin{itemize}
		\item initial $\mvba[s]$ with the following global predicate $Q_s$ as:
		
		$Q_s(\heights') \equiv$    (for each element $({\height}_j',\digest_j',\Sigma_{j}')$ of  input vector $\heights$, $\Vrfy( j||{\height}_j'||\digest_j',\Sigma_j) = \true$) $\wedge$ (exist at least $n-f$ distinct $j \in [n]$, such that $\height_j'>\agreed_j$)  $\wedge$ ($\forall$ $j \in [n]$, $\height_j'\ge\agreed_j$)
		
		\item wait for $\heights$ is updated, s.t. $\exists$ $n-f$ distinct $j \in [n]$, $\height_j>\agreed_j$:
		\begin{itemize}
			\item pass $\heights$ into $\mvba[s]$ as input
			\item wait for $\mvba[s]$ returns $\heights' := [({\height}_1',\digest_1',\Sigma_{1}'), \dots, ({\height}_n',\digest_n',\Sigma_{n}')]$ as output
			\begin{itemize}
				\item $\block_s \leftarrow \sort(\bigcup_{j \in [n]} \{\blocks[j][\agreed_j+1], \dots ,\blocks[j][\height_j'] \})$
				\item $\buf \leftarrow \buf \setminus \block_s$ and output $\block_s$
				\item for each $j \in [n]$, $\agreed_j \leftarrow {\height}_j'$
			\end{itemize}
		\end{itemize}
		
	\end{itemize}
	\end{itemize}


\noindent\textbf{Let} $\id$ (initialized as 1) be the session identification of $\mvba[\id]$, $Q$ of $\mvba$ be the following predicate:
%
$Q_\id[\{(1,s_1,\prf_{1,s_1}),\cdots, (n,s_n,\prf_{n,s_n})\}]\equiv$ (exist at least $n-f$ distinct $i \in [n]$, such that $s_i>\bar{s}_i$, and for each $i \in [n]$, $s_i\geq\bar{s}_i$  and $\Vrfy_{2f+1}(\langle \langle j, s_j \rangle,\hash(\payload_{j,s_j}) \rangle, \sigma_{j,s_j})=1$).

\begin{itemize}					
		\item	\textbf{while} $true$ {do} %for $\id=1,2,3,\cdots$
		\begin{itemize}		
				\item	upon waiting for $n-f$ distinct $(j,{s}_j,\prf_{j,{s}_j})$, s.t. $s_j >\bar{s}_j$, take $W$ as the $\MVBA[\id]$ input
				\item	 waiting for $\MVBA[\id]$ return $W'=\{(1,{s}_1',\prf_{1,{s}_1}'),\cdots, (n,{s}_n',\prf_{n,{s}_n}')\}$			
				
				\dotfill
				\begin{itemize}								
					%	\begin{tcolorbox}
						\item  $\blocks_1=\{\block[1,\bar{s}_1+1],\dots,\block[1,{s}_1']\}$,$\cdots$,$\blocks_n=\{\block[n,\bar{s}_n+1],\dots,\block[n,{s}_n']\}$
							
						\Comment{if ${s}_j'=\bar{s}_j$, then $\blocks_j=\emptyset$}
							
						\item for $1\leq j\leq n$
						
						\begin{itemize}		
								\item for	$\bar{s}_j+1\leq k\leq {s}_j'$,  if $\block[j,k]$ have not received yet, then $\callhelp(j,k)$			
						\end{itemize}	
					
						\item  $\log.append(\blocks_1,\cdots,\blocks_n)$ 		
						%	\end{tcolorbox}		
						
						\dotfill			
						\item   for any $(j,{s}_j,\prf_{j,{s}_j})\in W$, if ${s}_j<{s}_j'$, then $(j,{s}_j,\prf_{j,{s}_j})\leftarrow(1,{s}_1',\prf_{1,{s}_1}')$ 
							
						\Comment{ note that $W$ may continue to change as new $\block$ are received}
						\item $\widehat{W}\leftarrow W'$, $\id\leftarrow\id+1$
				\end{itemize}		
		\end{itemize}	
\end{itemize}	
	
\vspace{-0.2cm}				
\hrulefill

\begin{itemize}						
		\item	\textbf{Upon} $\MVBA[\id]$ return $W'=\{(1,{s}_1',\prf_{1,{s}_1}'),\cdots, (n,{s}_n',\prf_{n,{s}_n}')\}$
		\begin{itemize}		
				\item  $\blocks_1=\{\block[1,\bar{s}_1+1],\dots,\block[1,{s}_1']\}$,$\cdots$,$\blocks_n=\{\block[n,\bar{s}_n+1],\dots,\block[n,{s}_n']\}$
					
				\Comment{if ${s}_j'=\bar{s}_j$, then $\blocks_j=\emptyset$}					
				\item for $1\leq j\leq n$
				\begin{itemize}		
						\item for	$\bar{s}_j+1\leq k\leq {s}_j'$,  if $\block[j,k]$ have not received yet, then $\callhelp(j,k)$				
				\end{itemize}	
				\item  $\log.append(\blocks_1,\cdots,\blocks_n)$ 
		\end{itemize}	
\end{itemize}	
	
	
\end{tcolorbox}
\end{small}
\caption{The xdumbo protocol}
\label{alg:xdumbo}
\end{figure*}
	
	
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		
			
				
		










\ignore{

\subsection{Notarizable Weak Atomic Broadcast}
\subsection{}
	\begin{algorithm}			
		\begin{footnotesize}			
			\caption{$\XDUMBO$ protocol with identifier $\ID$ for $\node_i$}
		\begin{algorithmic}[1]
			\vspace*{0.1 cm}
			\State $\lv_k \leftarrow 0$ for $k \in [1,n]$
			\State $\lvs_k \leftarrow 0$ for $k \in [1,n]$
			\State $r \leftarrow 0$
			\State invoke $\abc_i$ as sender and participate in all other $\abc_j$ for $j \in [1, n]$
			\vspace*{0.1 cm}
			\Upon{delivering a valid $(tx, \Sigma_j)$ from $\abc_j$}
				\State $\lv_j \leftarrow \lv_j + 1 $
				\State $ \T_{ j, \lv_j} \leftarrow tx$
				\State $ \SIG_{ j, \lv_j} \leftarrow \Sigma_j $ 				
			\EndUpon
			\vspace*{0.1 cm}
			\Wait { for $n-f$ positions in $\lv$ grow from $\lvs$}
				\State activate $\MVBA_r$ with $\lv$ and $\SIG_{ j,\lv_j}$ for $j \in [1,n]$ as input				
			\EndWait
			\vspace*{0.1 cm}
			\Upon {delivering an output $\gv^r$ from $\MVBA_r$}
				\FOR {$j \in [1,n]$}
					\FOR {$k \in [\lvs_j+1,\gv^r_j]$}
						\IF {$\T_{j, k}$ not exists or  $\SIG_{j, k}$ is not valid}
							\State send a $\REQ([j,k])$ message to all parties
							\Wait { for receiving $f+1$ same $\SHARETX$ messages of $((j, k), tx, sig)$ from distinct parties}
								\State $\T_{j, k} \leftarrow tx$
								\State $\SIG_{j, k} \leftarrow sig$
							\EndWait
						\ENDIF				
						\State $block_r \leftarrow block_r \cup {{\T_{j, k}, \SIG_{j, k} }}$
					\ENDFOR
				\ENDFOR
				\State $\lvs \leftarrow \gv^r$
				\State $r \leftarrow r+1$
			\EndUpon
			\vspace*{0.1 cm}
			\Upon {receiving a $\REQ([j,k])$ message from $\node_l$}
				\IF {$\T_{j,k}$ exists}
					\State send $((j, k), \T_{j, k}, \SIG_{j, k})$ with a $\SHARETX$ message to $\node_l$
				\ENDIF
			\EndUpon
 `       			
		\end{algorithmic}
		\end{footnotesize}
	\end{algorithm}
}

==> callhelp.tex <==
%!TEX root = main.tex



The $\help$ service and the $\callhelp$ function are adapted from \cite{lu2021bolt}. As shown in Figure \ref{fig:help}, when a party realizes that it misses some $\payload$, it invokes the $\callhelp$ function to broadcast a $\ghlp$ message, which specifies some $\payload$ that shall be outputted but has not been received yet. 
The $\help$ service is a daemon process activated once every party is initialized and takes care of $\callhelp$ messages. If the $\callhelp$ function is invoked by some honest party, it can always successfully return the needed $\payload$, since at least $f+1$ honest parties have indeed received the outputted $\payload$ and they are also running a $\help$ daemon service to respond the request. The techniques of erasure-code and Merkle commitment tree  \cite{cachin2005asynchronous,miller2016honey} are used in the $\help$ daemon,  such that each $\help$ daemon only has to return a coded fragment of the fetched blocks, thus saving the communication complexity by an $\bigO(n)$ order.

\begin{figure}[ht]
	\vspace{-0.3cm}
	\begin{small}
	%	\centering
			\begin{tcolorbox}[
			colframe=gray!20,
			colback=gray!1,
			coltitle=gray!25!black,  
			fonttitle=\bfseries,
			adjusted title=CallHelp Function and Help Daemon  (for each node $\node_i$)]
				
				{\textbf{external function} $\callhelp(j, k)$:} 
				\begin{itemize}
					\item let $F\leftarrow[~ ]$ to be a dictionary structure such that $F[h]$ can store all leaves committed to Merkle tree root $h$ 
					\item multicast message $\ghlp(j, k)$
					\item upon receiving the message $\help(j, k, h, m_s, b_s)$ from node $\node_s$ for the first time:
					\begin{itemize}
						\item if $b_s$ is a valid Merkle branch for root $h$ and leaf $m_s$ then: $F[h] \leftarrow F[h] \cup (s, m_s) $;
						otherwise discard the   message
						\item if $|F[h]| = n-2f$ then:
						\begin{itemize}
							\item interpolate the $n-2f$ leaves stored in $F[h]$ to reconstruct $\blocks_j[k]$ %$M$, then parse $M$ as a sequence of $\block s$ and return $\block s$
						\end{itemize} 
					\end{itemize}					
				\end{itemize}
	\vspace{-0.2cm}
					\hrulefill
					\vspace{-0.2cm}
				\begin{center}
				{\bf	$\help$ daemon}
			\end{center}
					
					%process for node $\node_i$:
		%$\help$: It is a daemon process that can read the finalized output and it listens  to the down below event:
			%	\begin{itemize}
					 upon receiving message $\ghlp(j, k)$ from node $\node_s$ for the first time:
					\begin{itemize}
						\item wait for $\blocks_j[k]$ was record					
						\begin{itemize}
							\item let $\{m_k\}_{k \in [n]}$   be the fragements of a $(n-2f, n)$-erasure code   applied to $\blocks_j[k]$,  and $h$   be a Merkle tree root computed over $\{m_k\}_{k \in [n]}$ 
							\item send $\help(j,k, h, m_i, b_i)$ to  $\node_s$, where $m_i$ is the $i$-th erasure-code fragement of $\blocks_j[k]$  and $b_i$ is the $i$-th Merkle tree branch %MT branch rooted from $h$
						\end{itemize}
					\end{itemize}
			%	\end{itemize}
		
\end{tcolorbox}
		\caption{$\help$ is a daemon process that can read  the output of $\xdumbo$ and $\callhelp$ is a function used to call the $\help$ service}
		\label{fig:help}
	\end{small}
\vspace{-0.2cm}
\end{figure}





Remarks:  For some honest node $\node$, if the $\blocks_j[k]$ does not record, then $\blocks_j[k],\dots,\blocks_j[\height_j']$ all need to fetch according to the Figure \ref{alg:xdumbo}. Hence, he can broadcast $\ghlp$ message with batch way, and also the $\help$ messages can be sent with the batch way (at least $f+1$ honest nodes have received all these $\blocks_j$) if some honest nodes receive the batch $\ghlp$ message.
	












==> exp.tex <==
%!TEX root = main.tex

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

